Radiation hydrodynamics modeling of kilonovae with SNEC

We develop a method to compute synthetic kilonova light curves that combines numerical relativity simulations of neutron star mergers and the $\texttt{SNEC}$ radiation-hydrodynamics code. We describe our implementation of initial and boundary conditions, r-process heating, and opacities for kilonova simulations. We validate our approach by carefully checking that energy conservation is satisfied and by comparing the $\texttt{SNEC}$ results with those of two semi-analytic light curve models. We apply our code to the calculation of color light curves for three binaries having different mass ratios (equal and unequal mass) and different merger outcome (short-lived and long-lived remnants). We study the sensitivity of our results to hydrodynamic effects, nuclear physics uncertainties in the heating rates, and duration of the merger simulations. We find that hydrodynamics effects are typically negligible and that homologous expansion is a good approximation in most cases. However, pressure forces can amplify the impact of uncertainties in the radioactive heating rates. We also study the impact of shocks possibly launched into the outflows by a relativistic jet. None of our models match AT2017gfo, the kilonova in GW170817. This points to possible deficiencies in our merger simulations and kilonova models which neglect non-LTE effects and possible additional energy injection from the merger remnant, and to the need to go beyond the assumption of spherical symmetry adopted in this work.

==> Makefile <==
SRCS=KiloSNEC.tex
NAMES=$(SRCS:.tex=)
DOCS=$(SRCS:.tex=.pdf)

JUNK=.aux .bbl .blg .dvi .log .nav .out .ps .snm .tex.backup .toc Notes.bib

.PHONY: all bib clean veryclean

all: $(DOCS)

bib:
	@python fillbib.py \
	    --generate --journal_arXiv_fallback \
	    tex --bibtex references.bib $(SRCS)

$(DOCS): %.pdf: %.tex references.bib
	@pdflatex $<
	@python fillbib.py \
	    --generate --journal_arXiv_fallback \
	    tex --bibtex references.bib $<
	@bibtex $(<:.tex=)
	@pdflatex $<
	@pdflatex $<

clean:
	@for name in $(NAMES); do  \
		for ext in $(JUNK); do \
			rm -f $$name$$ext; \
		done;                  \
	done

veryclean: clean
	@rm -f $(DOCS)


==> Radiation hydrodynamics modeling of kilonovae with SNEC/Makefile <==
SRCS=KiloSNEC.tex
NAMES=$(SRCS:.tex=)
DOCS=$(SRCS:.tex=.pdf)

JUNK=.aux .bbl .blg .dvi .log .nav .out .ps .snm .tex.backup .toc Notes.bib

.PHONY: all bib clean veryclean

all: $(DOCS)

bib:
	@python fillbib.py \
	    --generate --journal_arXiv_fallback \
	    tex --bibtex references.bib $(SRCS)

$(DOCS): %.pdf: %.tex references.bib
	@pdflatex $<
	@python fillbib.py \
	    --generate --journal_arXiv_fallback \
	    tex --bibtex references.bib $<
	@bibtex $(<:.tex=)
	@pdflatex $<
	@pdflatex $<

clean:
	@for name in $(NAMES); do  \
		for ext in $(JUNK); do \
			rm -f $$name$$ext; \
		done;                  \
	done

veryclean: clean
	@rm -f $(DOCS)

